Quantile Bandits for Best Arms Identification

We consider a variant of the best arm identification task in stochastic multi-armed bandits. Motivated by risk-averse decision-making problems, our goal is to identify a set of $m$ arms with the highest $\tau$-quantile values within a fixed budget. We prove asymmetric two-sided concentration inequalities for order statistics and quantiles of random variables that have non-decreasing hazard rate, which may be of independent interest. With these inequalities, we analyse a quantile version of Successive Accepts and Rejects (Q-SAR). We derive an upper bound for the probability of arm misidentification, the first justification of a quantile based algorithm for fixed budget multiple best arms identification. We show illustrative experiments for best arm identification.

==> algorithm.tex <==
\section{Order Statistics Bandits Policy: OS-SAR}
\label{sec: quantile bandits OS-SAR}

\begin{algorithm}[t]
    \caption{OS-SAR}
    \label{alg:OS-SAR}
    \begin{algorithmic}
        \INPUT rank parameter $\tau$, arm set $\mathcal{K} = \{1,\dots, K\}$, number of arms to recommend $m$.
        \SET  Active set $\mathcal{A}_1= \mathcal{K}$, accepted set $\mathcal{M}_1 = \emptyset$, the number of arms left to find $l_1 = m$.
        $\overline{\log} (K) = \frac{1}{2} + \sum_{i = 2}^K \frac{1}{i}, n_0 = 0$, and for $p \in \{1, ..., K-1\},$
        $n_p = \left\lceil\frac{1}{\overline{\log }(K)} \frac{N-K}{K+1-p}\right\rceil.$
        \STATE \myz{fix the format}
        \FOR{each phase $p = 1,2, ..., K-1$:}
        \STATE  (1) For each $i \in \mathcal{A}_p$, sample arm $i$ for $n_p - n_{p-1}$ times.
        \STATE  (2) For each $i \in \mathcal{A}_p$, sort the $\lfloor \tau n_p \rfloor$ rank of order statistics $\hat{X}^\tau_{i, n_p}$ of arm $i$ in a non-increasing order, denote the sorted arms as $a_{best}, a_2, ..., a_{l_p}, a_{l_p+1}, ..., a_{worst}$ (with ties broken arbitrarily).
        \STATE  (3) Calculate $\widehat{\Delta}_{best} = \hat{X}^\tau_{a_{best}, n_p} - \hat{X}^\tau_{a_{l_p + 1}, n_p}$,
        $\widehat{\Delta}_{worst} =  \hat{X}^\tau_{a_{l_p}, n_p} - \hat{X}^\tau_{a_{worst}, n_p}$.
        % NOTE: should add l_p = |A_p| as well (in case l_p+1 out of range)
        \IF {$\widehat{\Delta}_{best} > \widehat{\Delta}_{worst}$} 
        % \COMMENT{$a_{best}$ is accepted.}
        % \STATE  {
        %move arm $a_{best}$ from active set to accepted set, i.e.
        \STATE  $\mathcal{A}_{p+1} = \mathcal{A}_{p} \backslash \{a_{best}\}$,
         $\mathcal{M}_{p + 1} = \mathcal{M}_{p} \cup \{a_{best}\}$,
         \STATE  $l_{p+1} = l_p -1$.
        %  }
        \ELSE
        % \COMMENT{$a_{worst}$ is rejected.}
            % \STATE  {
        % $a_{worst}$ is rejected, i.e.
         \STATE  $\mathcal{A}_{p+1} = \mathcal{A}_{p} \backslash \{a_{worst}\}$,
         $\mathcal{M}_{p + 1} = \mathcal{M}_{p},$
         \STATE  $l_{p+1} = l_p$.
        %  }
        \ENDIF
        \ENDFOR
        \STATE  Return the $m$ arms $\mathcal{S}_m^N = \mathcal{A}_{K-1} \cup \mathcal{M}_{K-1}$.
    \end{algorithmic}
  \end{algorithm}

%To address the problem that $\gamma_t$ needs to be tuned practically,
% With the objectives described in Section \ref{sec: Objectives and Assumptions},
We propose a Order Statistics based Successive Accepts and Rejects (OS-SAR) algorithm, which adapts the \textit{Successive Accepts and Rejects} (SAR) algorithm \citep{bubeck2013multiple}.
Recall that the goal is to recommend $m \geq 1$ out of $K$ arms with fixed budget, such that the probability of
error (Definition~\ref{defi: probability of error}) is minimized.
% The goal is to recommend a set of arms with size $m \geq 1$ with fixed budget, where the preference of arms is described according to
% a fixed level of quantiles.
% We formulated our objective in Eq. (\ref{defi: probability of error}), i.e. we aim to minimise the probability of error in terms of both simple regret
% and proxy simple regret.

We show OS-SAR in Algorithm \ref{alg:OS-SAR}.
Assume the total budget is at least $\frac{2K}{1-\tau}$,
which guarantees that after the initial round each arm has enough samples required by the concentration inequality in Section \ref{sec: concentration inequalities}.
% namely, n_1 >= 2/(1-\tau)
We divide the budget $N$ into $K-1$ phases.
The number of samples drawn for each arm in each phase remains the same as in the \citet{bubeck2013multiple}.
At each phase $p \in \{1, 2, \dots, K-1\}$, we maintain two sets (refer to Figure~\ref{fig: QSAR illustration.}):
i) the active set $\mathcal{A}_p$, which contains all arms that are actively drawn in phase $p$;
ii) the accepted set $\mathcal{M}_p$, which contains arms have been accepted.
% The active set is initialised as all arms $\mathcal{K}$.
In each phase $p$, an arm is removed from the active set, and it is either accepted or rejected.
The accepted arm is added into the accepted set.
At the end of phase $K-1$, only one arm remains in the active set.
The last remaining arm together with and the accepted set (containing $m-1$ arms) form the returned recommendation $\mathcal{S}_m^N$.

% \begin{figure}[t]
%   \centering
%   %\includegraphics[scale=0.4]{plots/Hist.pdf}
%   \includegraphics[scale=0.22]{plots/QSAR_plot.png}
%   \caption{Phase $p$ of OS-SAR illustration. Star indicates accepted arm, cross indicates rejected arm.
%     }
%     \label{fig: QSAR illustration.}
% \end{figure}

We introduce a simplified presentation of the SAR algorithm.
We can consider the task of identifying $m$ best arms as grouping arms into the optimal set $\mathcal{S}_m^\ast$ and non-optimal set.
Then intuitively it is easier to firstly group arms which are farther away from the boundary of the two groups,
since the estimation error is less likely to influence the grouping (Refer to Figure \ref{fig: QSAR illustration.}).
OS-SAR follows this intuition and determines to accept or reject the arm which is the farthest (based on estimations) from the boundary in each phase.
% The sub-optimality gap in Eq. (13) describes the gap/difference between each arm and the boundary.

Instead of considering all empirical gaps as SAR algorithm \citep{bubeck2013multiple} proposed,
OS-SAR decides whether to accept or reject an arm by only comparing two empirical gaps:
$\widehat{\Delta}_{best}$ and $\widehat{\Delta}_{worst}$ (defined in Algorithm \ref{alg:OS-SAR} step (3)).
This simplification also applies when using the mean as a summary statistic, and results in an equivalent algorithm to the original SAR in \citep{bubeck2013multiple}.
If $\widehat{\Delta}_{best} > \widehat{\Delta}_{worst}$, the arm with maximum empirical quantile is accepted;
otherwise, the arm with minimum empirical quantile is rejected.
% BAI tasks can be considered as partitioning arms into two set:
% the optimal (recommended) set $\mathcal{S}_m^\ast$,
% and the non-optimal set $\mathcal{K}/\mathcal{S}_m^\ast$.
% The arm with the largest empirical gap is most unlikely to be partitioned into a wrong set with imprecise estimations.
% So OS-SAR deals with the arm with largest empirical gap (i.e. $a_{best}, a_{worst}$) in each phase and makes the decision to accept or reject it.

When $m=1$, $\widehat{\Delta}_{worst} = \hat{Q}^\tau_{a_{best}} - \hat{Q}^\tau_{a_{worst}}$,
and $\widehat{\Delta}_{best} = \hat{Q}^\tau_{a_{best}} - \hat{Q}^\tau_{a_{2}}$. For all phases,
$\widehat{\Delta}_{worst} \geq \widehat{\Delta}_{best}$, thus OS-SAR will keep rejecting arms.
In this case, OS-SAR is the same as Q-SR (Algorithm \ref{alg:Q-SR}, shown in Section \ref{sec: experiment details}). %(shown in Appendix \ref{sec: experiment details}).

\paragraph{Theoretical analysis:}
% We now introduce the concept of \textit{gap}.
Recall optimality of arms are denoted as
$o_1, \dots, o_K$  s.t. $\mathbb{E}[X_{o_1, (k:N)}] \geq \dots \geq \mathbb{E}[X_{o_K, (k:N)}]$.
The optimal arm set of size $m$ is $\mathcal{S}_m^\ast = \{o_1, \dots, o_m\}$.
% Recall that $\mathcal{S}_m^{\ast}$ be the subset of the $m$ best arms,
% i.e. $i \in \mathcal{S}_m^\ast \text { iff } Q^\tau_{i} \geq Q^\tau_{(m)}$.
% In other words, $\mathcal{S}_m^\ast=\arg \max _{i \in \mathcal{K}}^{1 . . m} Q^\tau_{i}$.
For each arm $i \in \mathcal{K}$, we define the \textit{gap} $\Delta_i \geq 0$ by
$$
\Delta_{i} %= |\max _{k \neq i}^m Q^\tau_k - Q^\tau_i|
= \left\{\begin{array}{ll}
    \mathbb{E}[X_{i, (k:N)}]-\mathbb{E}[X_{o_{m+1}, (k:N)}] & \text { if } i \in  \mathcal{S}_m^\ast; \\
    \mathbb{E}[X_{o_m, (k:N)}]- \mathbb{E}[X_{i, (k:N)}] & \text { if } i \notin  \mathcal{S}_m^\ast.
\end{array}\right.
$$
We sort the gap in a non-decreasing order and denote the $i^{th}$ gap as $\Delta_{(i)}$,
i.e. $\Delta_{(1)} \leq \Delta_{(2)} \leq \dots \leq \Delta_{(K)}$.
The gaps characterise how separate the arms are and reflect the hardness of the problem.
The smaller the (minimum) gaps of the arms are, the harder the BAI task is.
We define the \textit{problem complexity} $H^{OS-SAR}$ as
%in terms of the gap, lower bound of hazard rate ($L$) and quantile level ($\tau$),
\begin{align}
  H^{OS-SAR} = \max_{i \in \{1, \dots, K\}} \frac{i}{L_H^2 \Delta^2_{(i)}
  \min\left\{\frac{1-\tau}{4 + L_H \Delta_{(i)}}, \frac{(1-\tau)^2}{8}\right\}}, \nonumber
\end{align}
where $L_H = \min_{i\in \mathcal{K}} L_i$  with $L_i$ as the lower bound of hazard rate of arm $i$.

In the following, we show an upper bound of the probability of error,
which depends on the problem complexity and has rate $\mathcal{O}(K^2 \exp{(\frac{-N + K}{\log K})})$ w.r.t the number of arms $K$ and budget $N$.
The smaller $H^{OS-SAR}$ is, the smaller the upper bound of error probability is.

% \textbf{Problem complexity:} Let $\Delta_{(i)}$ be the $i^{th}$ gap, i.e. $\Delta_{(1)} \leq \Delta_{(2)} \leq \dots \leq \Delta_{(K)}$, and $L_H = \min_{i \in \mathcal{K}} L_i$, we define the problem complexity with respect to OS-SAR as
% \begin{align}
% H^{OS-SAR} = \max_{i \in \{1, \dots, K\}} \frac{i}{1 - \tau} \left( \frac{4}{\Delta_{(i)}^2 L_H^2} + \frac{1}{\Delta_{(i)} L_H}\right)
% \end{align}

%This implies the hardness of the identifying $m$ optimal arms depends on $\Delta_{(m)} = \Delta_{(m+1)} = \min_{i \in \mathcal{S}_m^\ast} Q_i^\tau - \max_{j \notin \mathcal{S}_m^\ast} Q_j^\tau$, which is shown in the problem complexity below ($\{\Delta_{(m)}, \Delta_{(m+1)}\} \subset \min_{i \in \mathcal{K}} \Delta_i$). \textcolor{red}{check}
% \begin{restatable}[OS-SAR Proxy Simple Regret Upper Bound]{theo}{QSAR-P}
% \label{theo: QSAR proxy}
% The probability of error for OS-SAR satisfies
% \begin{align}
%     \delta = \mathbb{P}(R_{{\mathcal{S}_m}_N} > 0) \leq 2 K^2 \exp \left(- \frac{N-Kt_0}{16 \bar{\log}(K) H^{OS-SAR}}\right),
% \end{align}
% \end{restatable}

\begin{restatable}[OS-SAR Probability of Error Upper Bound]{theo}{QSAR}
  \label{theo: QSAR}
  The probability of error (Definition \ref{defi: probability of error}) for OS-SAR satisfies
  \begin{align}
    e_N \leq 2 K^2 \exp\left(- \frac{N-K}{16 \overline{\log}(K) H^{OS-SAR}} + C\right), \nonumber
     % \widetilde{\delta} = \mathbb{P}(\widetilde{R}_{{\mathcal{S}_m}_N} > 0) \leq 2 K^2 \exp \left(- \frac{N-Kt_0}{16 \bar{\log}(K) H^{OS-SAR}}\right),
  \end{align}
  where $C$ is the constant $(\frac{1}{4(1-\tau)} + \frac{b}{2\Delta_{(1)}}) \left(L_C^2 \Delta^2_{(K)} \max\{\frac{1-\tau}{4 + L_C \Delta_{(K)}}, \frac{(1-\tau)^2}{8}\}\right)$,
  with $L_C = \max_{i\in \mathcal{K}} L_i$, and $b$ is a positive constant. %specified in Theorem \ref{theo: link expected order statistics and population quantile}.
  \end{restatable}

% TODO: the constant term in the bound is larger (compared with the mean-based OS-SAR, when H is small), 
% and the bound could be very large (much bigger than 1) when N is not big enough.
% One way to possibly improve the constant is to instead of using lower bound of hazard rate, use hazard rate.

\begin{proof-sketch}
%We show the sketch of the proof for bandits results. %, which applies the concentration results shown in Section \ref{sec: concentration inequalities}.
Define the event $\xi$,
% and $\widetilde{\xi}$,
\begin{align}
%  \xi=  & \{\Forall  i \in\{1, \ldots, K\}, p \in\{1, \ldots, K-1\}, \nonumber \\
%   & \left| X^i_{(\lfloor n_p(1-\tau) \rfloor)} - \mathbb{E}[X^i_{(\lfloor n_p(1-\tau) \rfloor)}] \right| \leq \frac{1}{4} \Delta_{(K+1-p)}\}.\\
  \xi =& \{\forall i \in\{1, \ldots, K\}, p \in\{1, \ldots, K-1\}, \nonumber\\
  & \left| X_{i, (k(n_p):n_p)} - \mathbb{E}[X_{i, (k(N):N)}]\right| < \frac{1}{4} \Delta_{(K+1-p)}\}.
\end{align}
\textcolor{red}{fix notation.}
One can upper bound $\mathbb{P}(\bar{\xi})$, i.e. the probability that complementary event of $\xi$ happens,
%i.e.  and $\mathbb{P}(\widetilde{\xi})$,
by the union bound and the concentration results shown in Section \ref{sec: concentration inequalities}.
Then it suffices to show OS-SAR does not make any error on event $\xi$, %and $\widetilde{\xi}$,
and $\mathbb{P}(\bar{\xi})$ %and $1-\mathbb{P}(\widetilde{\xi})$
gives the probability of error shown in Theorem \ref{theo: QSAR}.

To show OS-SAR does not make any error on event $\xi$, %and $\widetilde{\xi}$,
we prove by induction on $p \geq 1$. We assume there is no wrong decision made in all previous $p-1$ phases.
This implies
(I) no arm from the optimal set is rejected and (II) no arm from non-optimal set is accepted.
For each of the two cases, we prove by contradiction,
that is, we assume that one arm from non-optimal set is accepted,
or one arm from optimal set is rejected in phase $p$.
\textcolor{red}{didn't define $\ell_i$}
These two assumptions give us
\begin{align}
  \Delta_{(K+1-p)} > & \max \{\mathbb{E}[X_{\ell_1, (k(N):N)}] - \mathbb{E}[X_{o_{m+1}, (k(N):N)}], \nonumber\\
 & \mathbb{E}[X_{o_m, (k(N):N)}] - \mathbb{E}[X_{\ell_{K+1-p}, (k(N):N)}]\}, \nonumber
\end{align}
which contradicts with the fact that $\Delta_{(K+1-p)} \leq \max \{\mathbb{E}[X_{\ell_1, (k(N):N)}] - \mathbb{E}[X_{o_{m+1}, (k(N):N)}], \mathbb{E}[X_{o_m, (k(N):N)}] - \mathbb{E}[X_{\ell_{K+1-p}, (k(N):N)}]\}$
since there are only $p-1$ arms that have been accepted or rejected at phase $p$.
For detailed proof, see Appendix \ref{sec: OS-SAR proof}.
\end{proof-sketch}


==> sections/related_work.tex <==
% !TEX root = ../icml2021_quantile_bandits.tex
\subsection{Related Work for Quantile Bandits}

    Mean-based best arm identification has been studied for fixed budget \citep{audibert2010best}
    and fixed confidence \citep{even2006action} settings.
    The difference between the two settings is how the exploration phase is terminated (when the budget runs out
    or when the quality of recommendations is at a fixed confidence level).
    We focus on the fixed budget setting for this work.
    \citet{audibert2010best} proposed the Successive Rejects algorithm for single best arm identification,
    which \citet{bubeck2013multiple} improved by proposing Successive Accepts and Rejects (SAR) algorithm for multiple arms.
    For a comprehensive review of bandits we refer to \citet{lattimore2018bandit}.
    % We will focus on related works which quantify arms using quantiles.

    In recent years, risk-averse decision-making has increasingly been studied,
    and quantiles have been shown to be an interesting summary statistic for bandit tasks.
    Previous work has considered the fixed confidence setting. For example,
    \citet{szorenyi2015qualitative} considered the case where the rewards are measured on a qualitative scale;
    % and addressed both best arm identification and regret minimisation setting.
    \citet{david_pure_2016} linked the quantile best arm identification problem with the max K-armed bandit problem \citep{david_max}; %under the fixed confidence setting.
    % They studied the fixed confidence setting under the PAC framework, providing a lower
    % bound on the sample complexity of any $(\epsilon, \delta)$-correct algorithm, and algorithms with matching upper bounds.
    \citet{yu2013sample} considered the problem of minimising
    risk measures including quantiles; % under the fixed confidence setting.
    \citet{howard_sequential_2019} studied the sequential estimation of quantiles and
    applied their concentration results to fixed confidence setting.
    % While optimising quantiles for bandits tasks have attracted lots of attentions,
    However, literature concerning quantile bandits with fixed budget is scarce.
    The most related work is \citet{tran-thanh_functional_2014}, which studied functional bandits, with quantiles as one example.
    They proposed the quantile based batch elimination algorithm.
    \citet{torossian_x-armed_2019} considered the fixed budget setting but focused on quantile optimization on stochastic black-box functions,
    which is different from our setting.

    \textbf{Comparison with Related Work:}
    % Q-SAR is adapted from the mean-based Successive Accepts and Rejects (SAR) algorithm \citep{bubeck2013multiple}.
    % The theoretical analysis performance for Q-SAR shown in Theorem \ref{theo: QSAR} is based on the proposed concentration inequalities in Section \ref{sec: concentration inequalities}.
    The upper bound of error probability of Q-SAR and SAR~\citep{bubeck2013multiple} have the same rate
    (in terms of the budget $N$ and number of arms $K$) up to constant factors.
    Our constant term is smaller when the minimum lower bound of hazard rate ($L_H$) takes a larger value.
    Unlike the mean-based algorithm, $H^\tau$ depends on the quantile level $\tau$ as well.
    The smaller $\tau$ is, the smaller the $H^\tau$ is. This can be intuitively explained as needing more samples to estimate higher level quantiles for IHR distributions. \\
    As far as we know, Q-SAR is the first policy designed to identify multiple arms with highest $\tau$-quantile values.
    The most related work is the functional bandits \citep{tran-thanh_functional_2014} where Batch Elimination (BE) is proposed for single best arm identification.
    They considered evaluating arms by various functionals of the reward distributions, including the quantile function.
    Since their concentration inequality is based on Chebyshev's inequality (and hence not exponential),
    the upper bound on the probability of error has rate $\mathcal{O}(K^2/N)$, which is slower than ours.



    % \citet{david_pac_nodate} considered the formulation of optimising cumulative rewards with a risk constraint,
    % i.e. $\lambda$-quantile of arms are larger than a threshold.
    % \citet{david_pure_2016} identified the arm for which the largest $\lambda$-quantile with the fixed confidence setting. They proposed the Max-Q algorithm which starts by sampling a fixed number of times from each arm and chooses the arm with a maximum $\lambda$-quantile estimated from the samples.
    % Their analysis focused on the sample complexity with uniformly sampling each arm.
    % They pointed out a risk-averse objective is nonlinear
    % and does not typically decompose into a sum over single period risks.
    % A special case of quantiles, the median have been applied in \textit{contaminated/corrupted bandits},
    % where an observant adversary that corrupts even a small fraction of the responses generated when arms are pulled \citep{kapoor_corruption-tolerant_2019, altschuler2019best}.

    % While most of risk-averse best arm identification works focus on single arm recommendation setting
    % \citep{szorenyi2015qualitative,david_pure_2016, david_pac_nodate},
    % \citet{yu2013sample} considered the multi-period risks ($m > 1$) for the fixed budget setting.
    % %Although they still considered the single best arm setting,
    % They addressed the problem of recommending $m$ arms after exploration phase (round $N$),
    % where objective function is formulated in terms of
    % the risk over the sum of recommendations,
    % i.e. \textit{the multi-period risk error} of a sequence of $m$ recommendations  $o_1,..., o_m \in \mathcal{S}_m^N$,
    % $$
    % \left| \max _{\left(A_{1}, \ldots, A_{m}\right) \in[K]^{m}}
    % Q^\tau\left(\sum_{s = 1}^{m} X^{A_s}_{s}\right)-Q^\tau\left(\sum_{s = 1}^{m} X_{s}^{o_s}\right) \right|.
    % $$
    % We formulate the multiple arm (i.e. set) simple regret (Definition \ref{defi: simple regret for set})
    % in a different way.
    % We consider the worst case simple regret we can get among the set,
    % while they considered the summary statistics over the sum of rewards.
    % For single period risk ($m=1$), the above definition is a special case (when $m = 1$) of
    % the arm simple regret (Definition \ref{defi: simple regret for arm}).
    % When summary statistics are nonlinear, the multiple period risk ($m > 1$)
    % does not typical decompose into a sum over single period risk.
    % Their objective notion is different from ours when $m > 1$.


==> sections/update_discussion.tex <==
\section{Note of changing rank}

This section includes note of what needs to be changed when Schanging rank as discussed in Remark \ref{remark: Single order statistic as quantiles estimator}.

\mengyan{Update Theorem \ref{theo: New Two-side Concentration inequality for quantiles.}}

\begin{restatable}[New Two-side Concentration Inequality for Quantiles]{theo}{TwosideBoundsQuantilesNew}
    \label{theo: Two-side Concentration inequality for quantiles.}
    Recall $v^r = \frac{2}{k L^2}$, $v^l = \frac{2(n-k+1)}{(k-1)^2 L^2}$, $c^r = \frac{2}{k L}, w_n = \frac{b}{n}$. %where $L$ is lower bound of hazard rate, $b > 0$ is a constant.
    For quantile level $\tau \in (0,1)$, let rank $k = \lfloor n(1-\tau) + 1 \rfloor$.
    Under Assumption \ref{ass:IHR} and \ref{ass: pdf continuously differentiable},
    % for \textcolor{red}{$n \geq \frac{2}{1 - \tau}$ do we need to make this assumption here?} and $\gamma \geq  0$,
    we have
    \begin{align}
    % \label{equ: new two-side Bernstein ine for quantiles right}
        \mathbb{P}\left( \hat{Q}^\tau_{n} - Q^\tau \geq \sqrt{2 v^r \gamma} + c^r \gamma + w_n \right) &\leq \exp(-\gamma). \nonumber \\
        %& \mathbb{P}\left(Q_\tau - \hat{Q}^\tau_{n} \geq   \sqrt{2v \gamma} + c \gamma \right) \leq e^{-\gamma}.
        \mathbb{P}\left( Q^\tau - \hat{Q}^\tau_{n} \geq \sqrt{2 v^l \gamma} + w_n \right) &\leq \exp(-\gamma). \nonumber
    \end{align}
\end{restatable}

\begin{proof}
    Denote the confidence interval for the right tail bound of order statistics as $d^r_{k, \gamma} = \sqrt{2 v^r \gamma} + c^r \gamma$.
    From Lemma \ref{lemma: concentration for Z_k}, we have $\mathbb{P}\left( X_{(k)} - \mathbb{E}[X_{(k)}] \geq d^r_{k, \gamma}  \right) \leq \exp(-\gamma)$.
    % Denote the confidence interval for the right tail bound of quantiles as $\widetilde{d}^r_{k, \gamma}$, we have
    % \begin{align}
    %     \mathbb{P}\left( \hat{Q}^\tau_{n} - Q^\tau \geq \widetilde{d}^r_{k, \gamma} \right) \leq \exp(-\gamma)
    % \end{align}
    With $k = \lfloor n(1-\tau) + 1\rfloor$, we have $\hat{Q}^\tau_n = X_{(k)}$ and from Theorem \ref{theo: link expected order statistics and population quantile},
    we have $\mathbb{E}[X_{(k)}] \leq Q^\tau + w_n$.
    With probability at least $1- \exp (-\gamma)$, the following event holds
    \begin{align}
         X_{(k)} - \mathbb{E}[X_{(k)}] < d^r_{k, \gamma}
         \Rightarrow X_{(k)} < \mathbb{E}[X_{(k)}] + d^r_{k, \gamma} \leq Q^\tau + w_n + d^r_{k, \gamma}
        \Rightarrow \hat{Q}^\tau_{n} - Q^\tau < w_n + d^r_{k, \gamma},
    \end{align}
    from which we have $\mathbb{P}(\hat{Q}^\tau_{n} - Q^\tau \geq w_n + d^r_{k, \gamma}) \leq \exp(-\gamma)$. % This concludes the proof.
% \end{proof}

% \LeftConQuant*

% \begin{proof}
    Denote the confidence interval for the right tail bound of order statistics as $d^l_{k, \gamma} = \sqrt{2 v^l \gamma}$.
    From Lemma \ref{lemma: new concentration for -Z_k}, we have $\mathbb{P}\left( \mathbb{E}[X_{(k)}] - X_{(k)} \geq d^l_{k, \gamma}  \right) \leq \exp(-\gamma)$.
    % Denote the confidence interval for the right tail bound of quantiles as $\widetilde{d}^r_{k, \gamma}$, we have
    % \begin{align}
    %     \mathbb{P}\left( \hat{Q}^\tau_{n} - Q^\tau \geq \widetilde{d}^r_{k, \gamma} \right) \leq \exp(-\gamma)
    % \end{align}
    With $k = \lfloor n(1-\tau) +1\rfloor$, we have $\hat{Q}^\tau_n = X_{(k)}$ and from Theorem \ref{theo: link expected order statistics and population quantile},
    we have $\mathbb{E}[X_{(k)}] \geq Q^\tau - w_n$.
    With probability at least $1- \exp (-\gamma)$, the following event holds
    \begin{align}
        \mathbb{E}[X_{(k)}] - X_{(k)} < d^l_{k, \gamma}
        \Rightarrow - X_{(k)} < - \mathbb{E}[X_{(k)}] + d^l_{k, \gamma} \leq - (Q^\tau - w_n)  + d^l_{k, \gamma}
        \Rightarrow  Q^\tau  - \hat{Q}^\tau_{n} < w_n + d^l_{k, \gamma},
    \end{align}
    from which we have $\mathbb{P}( Q^\tau  - \hat{Q}^\tau_{n} \geq w_n + d^l_{k, \gamma}) \leq \exp(-\gamma)$. This concludes the proof.
\end{proof}

\mengyan{Update Section \ref{sec: appendix re-express concentration}}
\subsection{New Re-expression of Concentration Results}
\label{sec: new appendix re-express concentration}

The proof of Q-SAR error bound uses the concentration results for quantiles.
We first further derive the result shown in Corollary \ref{coro: Rep Con Q} to show direct dependency on the number of samples $n$.
Recall the rank $k = \lfloor n(1-\tau) + 1 \rfloor$ with quantile level $\tau \in (0,1)$, which gives
\begin{align}
    \label{equ: new n range}
    n(1-\tau) < k \leq n(1-\tau) + 1.
\end{align}
We show the representation of concentration depending on $n$ in the following.

\begin{lemma}
    \label{lemma: new quantile concentration, dependency on n}
    For $\epsilon > 0$, recall $n$ denotes the number of samples,  $b$ is a constant depending on the density about $\tau$-quantile ($0<\tau<1$), $L$ is the lower bound of hazard rate.
    With $n \geq \frac{2}{1-\tau}$,
    Corollary \ref{coro: Rep Con Q}
    can be represented as
    \begin{align}
        & \mathbb{P}\left(\hat{Q}^\tau_{n} - Q^\tau \geq \epsilon \right) < \exp\left(-\frac{n (1-\tau)L^2 {\epsilon }^2}{2 (2 + 2L + b(1-\tau) L^2 \epsilon )}\right), \nonumber\\
        & \mathbb{P}\left( Q^\tau  - \hat{Q}^\tau_{n} \geq \epsilon \right) < \exp\left(-\frac{ n (1-\tau)L^2 {\epsilon }^2}{2 (\frac{8(1+\tau)}{1-\tau} + b (1-\tau) L^2 \epsilon )}\right). \nonumber
    \end{align}
    Combining the two bounds together, we have the two-sided bound shown in the following,
    \begin{align}
        \mathbb{P}\left(|\hat{Q}^\tau_{n} - Q^\tau| \geq \epsilon \right) < 2 \exp\left(-\frac{n (1-\tau)L^2 {\epsilon }^2}{2 (\alpha + \beta \epsilon )}\right), \nonumber
    \end{align}
    where $\alpha = \frac{8(1+\tau)}{1-\tau}, \beta = 2 L + b(1-\tau)L^2$.
\end{lemma}

\begin{proof}
    By assuming $n \geq \frac{2}{1-\tau}$, we have
    \begin{align}
        \label{eq:reason-n-geq-2}
        n(1-\tau) - 1 = n(1- (\tau + \frac{1}{n})) \geq \frac{1}{2} n (1-\tau).
    \end{align}

    Recall $v^r = \frac{2}{k L^2}$, $v^l = \frac{2(n-k+1)}{(k-1)^2 L^2}$, $c^r = \frac{2}{k L}, w_n = \frac{b}{n}$, we have
    \begin{align}
         \mathbb{P}\left(\hat{Q}^\tau_{n} - Q^\tau \geq \epsilon \right) &\leq \exp\left(-\frac{{\epsilon }^2}{2 (v^r+ (c^r + w_n) \epsilon )}\right)\\
         & = \exp\left(-\frac{{\epsilon }^2}{2 (\frac{2}{k L^2}+ (\frac{2}{k L} + \frac{b}{n}) \epsilon )}\right)\\
         &\leq \exp\left(-\frac{{\epsilon }^2}{2 (\frac{2}{k L^2}+ (\frac{2}{k L} + \frac{b (1-\tau)}{k}) \epsilon )}\right) && n \geq \frac{k}{1-\tau}\\
        \label{equ: new lemma 3 right proof last step with k}
         &= \exp\left(-\frac{k L^2 {\epsilon }^2}{2 (2+ (2L + b (1-\tau)L^2) \epsilon )}\right) \\
         &< \exp\left(-\frac{n (1-\tau) L^2 {\epsilon }^2}{2 (2+ (2L + b (1-\tau)L^2) \epsilon )}\right) && k > n (1-\tau)
    \end{align}
    Similarly,
    \begin{align}
        \mathbb{P}\left( Q^\tau  - \hat{Q}^\tau_{n} \geq \epsilon \right) &\leq \exp\left(- \frac{{\epsilon } ^ 2}{2 (v^l + w_n \epsilon)}\right)\\
        \label{equ: new lemma 3 left proof last step with k}
        & = \exp\left(- \frac{{\epsilon } ^ 2}{2 (\frac{2(n-k+1)}{(k-1)^2 L^2} + \frac{b}{n} \epsilon)}\right)\\
        & < \exp\left(- \frac{{\epsilon } ^ 2}{2 (\frac{2(1+\tau)}{1/4 n(1-\tau)^2 L^2} + \frac{b}{n} \epsilon)}\right)&& k - 1 > \frac{n(1-\tau)}{2}, \frac{1}{n} \leq 1\\
        & = \exp\left(- \frac{{1/4 n (1-\tau)^2 L^2  \epsilon } ^ 2}{2 (2(1+\tau) + 1/4 b (1-\tau)^2 L^2 \epsilon)}\right)\\
        & = \exp\left(- \frac{{ n (1-\tau) L^2  \epsilon } ^ 2}{2 (\frac{8(1+\tau)}{1-\tau} +  b (1-\tau) L^2 \epsilon)}\right).
    \end{align}

Then let $\alpha = \max\{2, \frac{8(1+\tau)}{1-\tau}\} = \frac{8(1+\tau)}{1-\tau}, \beta = \max\{2 L + b(1-\tau)L^2,  b (1-\tau) L^2\} = 2 L + b(1-\tau)L^2$,
% one can possibly make the constant \frac{8(1+\tau)}{1-\tau} smaller by assuming n < 1/(c-1)\tau, where c > 1 and is very close to 1. Then we have the constant as 8 c \tau\ (1-\tau)
we have
\begin{align}
    \mathbb{P}\left(|\hat{Q}^\tau_{n} - Q^\tau| \geq \epsilon \right) & = \mathbb{P}\left(\hat{Q}^\tau_{n} - Q^\tau \geq \epsilon \right) + \mathbb{P}\left( Q^\tau  - \hat{Q}^\tau_{n} \geq \epsilon \right) \nonumber\\
    & < 2 \exp\left(-\frac{n (1-\tau)L^2 {\epsilon }^2}{2 (\alpha + \beta \epsilon )}\right). \nonumber
\end{align}

\end{proof}

\begin{remark}[Lower bound of sample size]
    In Lemma \ref{lemma: new quantile concentration, dependency on n}, we make an assumption about the lower bound of sample size, i.e. $n \geq \frac{2}{1-\tau}$.
    Note that along with the left inequality of  Equation~(\ref{equ: new n range}), the lower bound of sample size can be expressed as $n \geq \frac{\max\{k,2\}}{1-\tau}$. When $k\geq2$, we have $n \geq \frac{k}{1-\tau}$, which holds for all $n\geq 1$.
    This implies that instead of making an assumption about sample size $n$, we could equivalently
    make an assumption about the rank ($k \geq 2$) or the quantile level
    ($\tau \leq 1 - \frac{2}{n}$ with $n \geq 2$).\\
    Note the constant 2 in $n \geq \frac{2}{1-\tau}$ is chosen to have a simpler expression for the concentration bounds,
    one can choose any constant bigger than 1 (such that the term $n(1-\tau) - 1$
    is valid in Equation~(\ref{eq:reason-n-geq-2})).
\end{remark}

\mengyan{Note the definition of $\alpha, \beta_i$ in the definition of $H^\tau$ (Eq. \ref{equ: problem complexity H}) should be changed accordingly, i.e. $\alpha =  = \frac{8(1+\tau)}{1-\tau}, \beta_i =  2 L_i + b(1-\tau)L_i^2$}

We show a variant of Lemma \ref{lemma: new quantile concentration, dependency on n} where we
remove the lower bound assumption of the number of samples.
The derived concentration bounds have a constant term, which does not influence the convergence rate in terms of $n$.
\mengyan{to be updated}


\section{Note of proof methods of Theorem \ref{theo: link expected order statistics and population quantile}}

\begin{defi}[H-bounded transforms \cite{Blom1958} Section 3.5]
    Let $H(u; a,b)$ be defined by 
    \begin{align}
        H(u ; a, b)=u^a(1-u)^b,
    \end{align}
    where $a,b$ are two constants. 
    A transform $G(u)$ is called H-bounded, if exists $a$ and $b$ such that $G(u)H(u;a,b)$ is bounded for $0 \leq u \leq 1$. 
\end{defi}

\begin{theo}[$\alpha, \beta-$corrections \cite{Blom1958} Theorem 6.2.]
    \label{theo: alpha-beta correction}
    \begin{align}
        \mathrm{E}\left(X_{(r)}\right)=Q\left(\pi_r\right)+R\\
        \label{equ: alpha-beta correction pi}
        \text{with } \pi_r=\frac{\left(n-r+1-\alpha_r\right)}{\left(n+1-\alpha_r-\beta_r\right)}
    \end{align}
    We assume $Q(u)$ is H-bounded, $Q(u)$ and $Q^{\prime}(u)$ are bounded and continuous (\mengyan{etc}).
    For $a \leq \alpha_r < n-r+1, b\leq \beta_r < r$, and $\alpha_r \rightarrow 0$ when $(n-r+1)/n \rightarrow 0$, $\beta_r \rightarrow 0$ when $(n-r+1)/n \rightarrow 1$,
    then \[R = \mathcal{O} (\frac{1}{n})\]
\end{theo}

\begin{theo}[Link expected order statistics and population quantile \cite{david_order_1981}]
    \label{updated theo: link expected order statistics and population quantile}
    Under Assumption \ref{ass: pdf continuously differentiable},
    there exists constant $b \geq 0$ and scalars $w_n$ such that % $w_n = \frac{b \tau(1- \tau)}{2(n+2)}$, then
    $w_n = \frac{b}{n}$, then
    $|\mathbb{E}[X_{(k)}] - Q^\tau| \leq w_n$, where $k = \lfloor n(1-\tau) + 1 \rfloor$.
    % $Q^\tau - w_n \leq \mathbb{E}[X_{(\lfloor n(1-\tau) \rfloor}] \leq Q^\tau + w_n.$
\end{theo}

\mengyan{An alternative approach is to go with Theorem \ref{theo: alpha-beta correction}}
% That is, we select $r = \lfloor n(1-\pi_r) + 1 \rfloor$.
From Eq. (\ref{equ: alpha-beta correction pi}), we have 
\begin{align}
    k = n(1-\tau) + 1 - \alpha_k - \tau + \tau \alpha_k + \tau \beta_k
\end{align}
Questions:
\begin{itemize}
    \item are the conditions in Theorem \ref{theo: alpha-beta correction} satisfied in our case? \\
    \item can we get $k = \lfloor n(1-\tau) + 1 \rfloor$ for valid $\alpha_k, \beta_k$? \\
    since $n(1-\tau) \leq \lfloor n(1-\tau) + 1 \rfloor \leq n(1-\tau) + 1$, we need to find $\alpha_k, \beta_k$ such that 
    $-1 \leq \tau (\alpha_k + \beta_k -1) - \alpha_k \leq 0$.
    Our quantile distributions seem to be AL-transforms (e.g. inverse function of normal, gamma, exponential, Laplace)? This gives $a, b>0$. 
    Note we actually need $- \tau + \tau \alpha_k + \tau \beta_k$ to be reminder term of $n\tau$. If we have a more strict condition that $- \tau + \tau \alpha_k + \tau \beta_k$ can be mapping to any value between -1 and 0 by selecting suitable $\alpha_k, \beta_k$, this can be proved as well. \\
    This might also work for our orginal rank $k = \lfloor n(1-\tau)\rfloor$.
    \item Big O notation: $|\mathbb{E}[X_{(k)}] - Q^\tau | \leq \frac{b}{n}$ for all $n > n_0$.
\end{itemize}

\begin{lemma}[Expected order statistics products \citet{david_order_1981} Eq. (3.1.6)]
    \label{lemma: Expected order statistics products}
    For order statistics $X_{(r_i)} (i=1, \dots, k)$ with sample size $n$, the expected products of order statistics is 
    \begin{align}
        \mathrm{E}\left(\prod_{i=1}^k X_{(r_i)}^{a_i}\right)=\frac{n !}{\left(n+\sum_{i=1}^k a_i\right) !} \prod_{i=1}^k \frac{\left(r_i-1+\sum_{j=1}^i a_j\right) !}{\left(r_i-1+\sum_{j=1}^{i-1} a_j\right) !} .
    \end{align}
\end{lemma}

\begin{coro}[\citet{david_order_1981} Eq. (3.1.7)]
    \label{coro: Expected order statistics products}
    From Lemma \ref{lemma: Expected order statistics products}, and set $p_r = \frac{n-r+1}{n+1}, q_r = 1-p_r$, we have 
    \begin{align}
        \mathbb{E}[X_{(r)}] &= p_r,\\
        \mathbb{E}\left[\left(X_{(r)} - \mathbb{E}[X_{(r)}]\right)^2\right] &= \frac{p_r q_r}{n+2};\\
        \mathbb{E}\left[\left(X_{(r)} - \mathbb{E}[X_{(r)}]\right)^3\right] &= \frac{2 p_r\left(q_r-p_r\right) q_r}{(n+2)(n+3)}.
    \end{align}
\end{coro}
